PA-CFL: Privacy-Adaptive Clustered Federated Learning for Transformer-Based Sales Forecasting on Heterogeneous Retail Data

Federated learning (FL) enables retailers to share model parameters for demand forecasting while maintaining privacy. However, heterogeneous data across diverse regions, driven by factors such as varying consumer behavior, poses challenges to the effectiveness of federated learning. To tackle this challenge, we propose Privacy-Adaptive Clustered Federated Learning (PA-CFL) tailored for demand forecasting on heterogeneous retail data. By leveraging differential privacy and feature importance distribution, PA-CFL groups retailers into distinct ``bubbles'', each forming its own federated learning system to effectively isolate data heterogeneity. Within each bubble, Transformer models are designed to predict local sales for each client. Our experiments demonstrate that PA-CFL significantly surpasses FedAvg and outperforms local learning in demand forecasting performance across all participating clients. Compared to local learning, PA-CFL achieves a 5.4% improvement in R^2, a 69% reduction in RMSE, and a 45% decrease in MAE. Our approach enables effective FL through adaptive adjustments to diverse noise levels and the range of clients participating in each bubble. By grouping participants and proactively filtering out high-risk clients, PA-CFL mitigates potential threats to the FL system. The findings demonstrate PA-CFL's ability to enhance federated learning in time series prediction tasks with heterogeneous data, achieving a balance between forecasting accuracy and privacy preservation in retail applications. Additionally, PA-CFL's capability to detect and neutralize poisoned data from clients enhances the system's robustness and reliability.

==> tables/sensitivity.tex <==
\begin{table}[h]
\centering
\caption{Sensitivity for Different Regions}
\small
\begin{tabular}{|c|c|}
\hline
\textbf{Region} & \textbf{Sensitivity} \\ \hline
Southeast Asia      & 0.0651  \\ \hline
South Asia          & 0.0526  \\ \hline
Oceania             & 0.0268  \\ \hline
Eastern Asia        & 0.0515  \\ \hline
West of USA         & 0.0163  \\ \hline
US Center           & 0.0195  \\ \hline
West Africa         & 0.0138  \\ \hline
North Africa        & 0.0184  \\ \hline
Western Europe      & 0.0356  \\ \hline
Central America     & 0.0185  \\ \hline
South America       & 0.0227  \\ \hline
Southern Europe     & 0.0607  \\ \hline
East of USA         & 0.0093  \\ \hline
South of USA        & 0.0204  \\ \hline
\end{tabular}
\label{tab:sensitivity_regions}
\end{table}

